Reweighting Improves Conditional Risk Bounds

In this work, we study the weighted empirical risk minimization (weighted ERM) schema, in which an additional data-dependent weight function is incorporated when the empirical risk function is being minimized. We show that under a general ``balanceable" Bernstein condition, one can design a weighted ERM estimator to achieve superior performance in certain sub-regions over the one obtained from standard ERM, and the superiority manifests itself through a data-dependent constant term in the error bound. These sub-regions correspond to large-margin ones in classification settings and low-variance ones in heteroscedastic regression settings, respectively. Our findings are supported by evidence from synthetic data experiments.

==> main-arXiv.bbl.tex <==
\begin{thebibliography}{}

\bibitem[\protect\citeauthoryear{Ausset, Cl{\'e}men{\c{c}}on, and Portier}{Ausset et~al.}{2022}]{ausset2022empirical}
Ausset, G., S.~Cl{\'e}men{\c{c}}on, and F.~Portier (2022).
\newblock Empirical risk minimization under random censorship.
\newblock {\em Journal of Machine Learning Research\/}.

\bibitem[\protect\citeauthoryear{Awasthi, Mao, Mohri, and Zhong}{Awasthi et~al.}{2022}]{awasthi2022h}
Awasthi, P., A.~Mao, M.~Mohri, and Y.~Zhong (2022).
\newblock H-consistency bounds for surrogate loss minimizers.
\newblock In {\em International Conference on Machine Learning}, pp.\  1117--1174. PMLR.

\bibitem[\protect\citeauthoryear{Bach}{Bach}{2010}]{bach2010self}
Bach, F. (2010).
\newblock Self-concordant analysis for logistic regression.
\newblock {\em Electronic Journal of Statistics\/}~{\em 4}, 384--414.

\bibitem[\protect\citeauthoryear{Bartlett, Bousquet, and Mendelson}{Bartlett et~al.}{2005}]{bartlett2005local}
Bartlett, P.~L., O.~Bousquet, and S.~Mendelson (2005).
\newblock Local rademacher complexities.
\newblock {\em The Annals of Statistics\/}~{\em 33\/}(4), 1497--1537.

\bibitem[\protect\citeauthoryear{Bartlett and Mendelson}{Bartlett and Mendelson}{2006}]{bartlett2006empirical}
Bartlett, P.~L. and S.~Mendelson (2006).
\newblock Empirical minimization.
\newblock {\em Probability theory and related fields\/}~{\em 135\/}(3), 311--334.

\bibitem[\protect\citeauthoryear{Bartlett and Wegkamp}{Bartlett and Wegkamp}{2008}]{bartlett2008classification}
Bartlett, P.~L. and M.~H. Wegkamp (2008).
\newblock Classification with a reject option using a hinge loss.
\newblock {\em Journal of Machine Learning Research\/}~{\em 9\/}(8).

\bibitem[\protect\citeauthoryear{Boucheron, Bousquet, and Lugosi}{Boucheron et~al.}{2005}]{boucheron2005theory}
Boucheron, S., O.~Bousquet, and G.~Lugosi (2005).
\newblock Theory of classification: A survey of some recent advances.
\newblock {\em ESAIM: probability and statistics\/}~{\em 9}, 323--375.

\bibitem[\protect\citeauthoryear{Bousquet, Boucheron, and Lugosi}{Bousquet et~al.}{2003}]{bousquet2003introduction}
Bousquet, O., S.~Boucheron, and G.~Lugosi (2003).
\newblock Introduction to statistical learning theory.
\newblock In {\em Summer school on machine learning}, pp.\  169--207. Springer.

\bibitem[\protect\citeauthoryear{Bousquet and Zhivotovskiy}{Bousquet and Zhivotovskiy}{2021}]{bousquet2021fast}
Bousquet, O. and N.~Zhivotovskiy (2021).
\newblock Fast classification rates without standard margin assumptions.
\newblock {\em Information and Inference: A Journal of the IMA\/}~{\em 10\/}(4), 1389--1421.

\bibitem[\protect\citeauthoryear{Cawley, Talbot, Foxall, Dorling, and Mandic}{Cawley et~al.}{2004}]{cawley2004heteroscedastic}
Cawley, G.~C., N.~L. Talbot, R.~J. Foxall, S.~R. Dorling, and D.~P. Mandic (2004).
\newblock Heteroscedastic kernel ridge regression.
\newblock {\em Neurocomputing\/}~{\em 57}, 105--124.

\bibitem[\protect\citeauthoryear{Chow}{Chow}{1970}]{chow1970optimum}
Chow, C. (1970).
\newblock On optimum recognition error and reject tradeoff.
\newblock {\em IEEE Transactions on information theory\/}~{\em 16\/}(1), 41--46.

\bibitem[\protect\citeauthoryear{Cortes, DeSalvo, and Mohri}{Cortes et~al.}{2016}]{cortes2016learning}
Cortes, C., G.~DeSalvo, and M.~Mohri (2016).
\newblock Learning with rejection.
\newblock In {\em Algorithmic Learning Theory: 27th International Conference, ALT 2016, Bari, Italy, October 19-21, 2016, Proceedings 27}, pp.\  67--82. Springer.

\bibitem[\protect\citeauthoryear{Cortes, Mansour, and Mohri}{Cortes et~al.}{2010}]{cortes2010learning}
Cortes, C., Y.~Mansour, and M.~Mohri (2010).
\newblock Learning bounds for importance weighting.
\newblock {\em Advances in neural information processing systems\/}~{\em 23}.

\bibitem[\protect\citeauthoryear{Cortes, Mohri, Riley, and Rostamizadeh}{Cortes et~al.}{2008}]{cortes2008sample}
Cortes, C., M.~Mohri, M.~Riley, and A.~Rostamizadeh (2008).
\newblock Sample selection bias correction theory.
\newblock In {\em Algorithmic Learning Theory: 19th International Conference, ALT 2008, Budapest, Hungary, October 13-16, 2008. Proceedings 19}, pp.\  38--53. Springer.

\bibitem[\protect\citeauthoryear{Daye, Chen, and Li}{Daye et~al.}{2012}]{daye2012high}
Daye, Z.~J., J.~Chen, and H.~Li (2012).
\newblock High-dimensional heteroscedastic regression with an application to eqtl data analysis.
\newblock {\em Biometrics\/}~{\em 68\/}(1), 316--326.

\bibitem[\protect\citeauthoryear{Diakonikolas, Gouleakis, and Tzamos}{Diakonikolas et~al.}{2019}]{diakonikolas2019distribution}
Diakonikolas, I., T.~Gouleakis, and C.~Tzamos (2019).
\newblock Distribution-independent pac learning of halfspaces with massart noise.
\newblock {\em Advances in Neural Information Processing Systems\/}~{\em 32}.

\bibitem[\protect\citeauthoryear{Diakonikolas, Park, and Tzamos}{Diakonikolas et~al.}{2021}]{diakonikolas2021relu}
Diakonikolas, I., J.~H. Park, and C.~Tzamos (2021).
\newblock Relu regression with massart noise.
\newblock {\em Advances in Neural Information Processing Systems\/}~{\em 34}, 25891--25903.

\bibitem[\protect\citeauthoryear{Dudley}{Dudley}{2014}]{dudley2014uniform}
Dudley, R.~M. (2014).
\newblock {\em Uniform central limit theorems}, Volume 142.
\newblock Cambridge university press.

\bibitem[\protect\citeauthoryear{El-Yaniv et~al.}{El-Yaniv et~al.}{2010}]{noisefree_ro_2010_JMLR}
El-Yaniv, R. et~al. (2010).
\newblock On the foundations of noise-free selective classification.
\newblock {\em JMLR\/}~{\em 11\/}(5).

\bibitem[\protect\citeauthoryear{Franc, Prusa, and Voracek}{Franc et~al.}{2023}]{franc2023optimal}
Franc, V., D.~Prusa, and V.~Voracek (2023).
\newblock Optimal strategies for reject option classifiers.
\newblock {\em Journal of Machine Learning Research\/}~{\em 24\/}(11), 1--49.

\bibitem[\protect\citeauthoryear{Ge, Tang, Fan, Ma, and Jin}{Ge et~al.}{2023}]{ge2023maximum}
Ge, J., S.~Tang, J.~Fan, C.~Ma, and C.~Jin (2023).
\newblock Maximum likelihood estimation is all you need for well-specified covariate shift.
\newblock {\em arXiv preprint arXiv:2311.15961\/}.

\bibitem[\protect\citeauthoryear{Hanczar and Dougherty}{Hanczar and Dougherty}{2008}]{hanczar2008classification}
Hanczar, B. and E.~R. Dougherty (2008).
\newblock Classification with reject option in gene expression data.
\newblock {\em Bioinformatics\/}~{\em 24\/}(17), 1889--1895.

\bibitem[\protect\citeauthoryear{Hanneke}{Hanneke}{2009}]{hanneke2009theoretical}
Hanneke, S. (2009).
\newblock {\em Theoretical foundations of active learning}.
\newblock Carnegie Mellon University.

\bibitem[\protect\citeauthoryear{Haussler}{Haussler}{1995}]{haussler1995sphere}
Haussler, D. (1995).
\newblock Sphere packing numbers for subsets of the boolean n-cube with bounded {Vapnik-Chervonenkis} dimension.
\newblock {\em Journal of Combinatorial Theory, Series A\/}~{\em 69\/}(2), 217--232.

\bibitem[\protect\citeauthoryear{Herbei and Wegkamp}{Herbei and Wegkamp}{2006}]{herbei2006classification}
Herbei, R. and M.~H. Wegkamp (2006).
\newblock Classification with reject option.
\newblock {\em The Canadian Journal of Statistics/La Revue Canadienne de Statistique\/}, 709--721.

\bibitem[\protect\citeauthoryear{Jiang and Li}{Jiang and Li}{2016}]{jiang2016doubly}
Jiang, N. and L.~Li (2016).
\newblock Doubly robust off-policy value evaluation for reinforcement learning.
\newblock In {\em International Conference on Machine Learning}, pp.\  652--661. PMLR.

\bibitem[\protect\citeauthoryear{Kanade, Rebeschini, and Vaskevicius}{Kanade et~al.}{2022}]{kanade2022exponential}
Kanade, V., P.~Rebeschini, and T.~Vaskevicius (2022).
\newblock Exponential tail local rademacher complexity risk bounds without the bernstein condition.
\newblock {\em arXiv preprint arXiv:2202.11461\/}.

\bibitem[\protect\citeauthoryear{Kendall and Gal}{Kendall and Gal}{2017}]{kendall2017uncertainties}
Kendall, A. and Y.~Gal (2017).
\newblock What uncertainties do we need in bayesian deep learning for computer vision?
\newblock {\em Advances in neural information processing systems\/}~{\em 30}.

\bibitem[\protect\citeauthoryear{Klein and Young}{Klein and Young}{2015}]{klein2015number}
Klein, P. and N.~E. Young (2015).
\newblock On the number of iterations for dantzig--wolfe optimization and packing-covering approximation algorithms.
\newblock {\em SIAM Journal on Computing\/}~{\em 44\/}(4), 1154--1172.

\bibitem[\protect\citeauthoryear{Klochkov and Zhivotovskiy}{Klochkov and Zhivotovskiy}{2021}]{klochkov2021stability}
Klochkov, Y. and N.~Zhivotovskiy (2021).
\newblock Stability and deviation optimal risk bounds with convergence rate $ o (1/n) $.
\newblock {\em Advances in Neural Information Processing Systems\/}~{\em 34}, 5065--5076.

\bibitem[\protect\citeauthoryear{Kohler and Langer}{Kohler and Langer}{2021}]{kohler2021rate}
Kohler, M. and S.~Langer (2021).
\newblock On the rate of convergence of fully connected deep neural network regression estimates.
\newblock {\em The Annals of Statistics\/}~{\em 49\/}(4), 2231--2249.

\bibitem[\protect\citeauthoryear{Koltchinskii and Panchenko}{Koltchinskii and Panchenko}{2000}]{koltchinskii2000rademacher}
Koltchinskii, V. and D.~Panchenko (2000).
\newblock Rademacher processes and bounding the risk of function learning.
\newblock In {\em High dimensional probability II}, pp.\  443--457. Springer.

\bibitem[\protect\citeauthoryear{Koren and Levy}{Koren and Levy}{2015}]{koren2015fast}
Koren, T. and K.~Levy (2015).
\newblock Fast rates for exp-concave empirical risk minimization.
\newblock {\em Advances in Neural Information Processing Systems\/}~{\em 28}.

\bibitem[\protect\citeauthoryear{Lakshminarayanan, Pritzel, and Blundell}{Lakshminarayanan et~al.}{2017}]{lakshminarayanan2017simple}
Lakshminarayanan, B., A.~Pritzel, and C.~Blundell (2017).
\newblock Simple and scalable predictive uncertainty estimation using deep ensembles.
\newblock {\em Advances in Neural Information Processing Systems\/}~{\em 30}.

\bibitem[\protect\citeauthoryear{Lee, Bartlett, and Williamson}{Lee et~al.}{1996}]{lee1996importance}
Lee, W.~S., P.~L. Bartlett, and R.~C. Williamson (1996).
\newblock The importance of convexity in learning with squared loss.
\newblock In {\em Proceedings of the Ninth Annual Conference on Computational Learning Theory}, pp.\  140--146.

\bibitem[\protect\citeauthoryear{Liang, Rakhlin, and Sridharan}{Liang et~al.}{2015}]{liang2015learning}
Liang, T., A.~Rakhlin, and K.~Sridharan (2015).
\newblock Learning with square loss: Localization through offset rademacher complexity.
\newblock In {\em Conference on Learning Theory}, pp.\  1260--1285. PMLR.

\bibitem[\protect\citeauthoryear{Mammen and Tsybakov}{Mammen and Tsybakov}{1999}]{mammen1999smooth}
Mammen, E. and A.~B. Tsybakov (1999).
\newblock Smooth discrimination analysis.
\newblock {\em The Annals of Statistics\/}~{\em 27\/}(6), 1808--1829.

\bibitem[\protect\citeauthoryear{Mao, Mohri, and Zhong}{Mao et~al.}{2023}]{mao2023h}
Mao, A., M.~Mohri, and Y.~Zhong (2023).
\newblock $ h $-consistency bounds: Characterization and extensions.
\newblock In {\em Thirty-seventh Conference on Neural Information Processing Systems}.

\bibitem[\protect\citeauthoryear{Massart and N{\'e}d{\'e}lec}{Massart and N{\'e}d{\'e}lec}{2006}]{massart2006risk}
Massart, P. and {\'E}.~N{\'e}d{\'e}lec (2006).
\newblock Risk bounds for statistical learning.
\newblock {\em The Annals of Statistics\/}~{\em 34\/}(5), 2326--2366.

\bibitem[\protect\citeauthoryear{Mendelson}{Mendelson}{2002a}]{mendelson2002improving}
Mendelson, S. (2002a).
\newblock Improving the sample complexity using global data.
\newblock {\em IEEE transactions on Information Theory\/}~{\em 48\/}(7), 1977--1991.

\bibitem[\protect\citeauthoryear{Mendelson}{Mendelson}{2002b}]{mendelson2002rademacher}
Mendelson, S. (2002b).
\newblock Rademacher averages and phase transitions in glivenko-cantelli classes.
\newblock {\em IEEE transactions on Information Theory\/}~{\em 48\/}(1), 251--263.

\bibitem[\protect\citeauthoryear{Mendelson}{Mendelson}{2018}]{mendelson2018learning}
Mendelson, S. (2018).
\newblock Learning without concentration for general loss functions.
\newblock {\em Probability Theory and Related Fields\/}~{\em 171\/}(1-2), 459--502.

\bibitem[\protect\citeauthoryear{Min, Wang, Zhou, and Gu}{Min et~al.}{2021}]{min2021variance}
Min, Y., T.~Wang, D.~Zhou, and Q.~Gu (2021).
\newblock Variance-aware off-policy evaluation with linear function approximation.
\newblock {\em Advances in neural information processing systems\/}~{\em 34}, 7598--7610.

\bibitem[\protect\citeauthoryear{Mozannar and Sontag}{Mozannar and Sontag}{2020}]{mozannar2020consistent}
Mozannar, H. and D.~Sontag (2020).
\newblock Consistent estimators for learning to defer to an expert.
\newblock In {\em International Conference on Machine Learning}, pp.\  7076--7087. PMLR.

\bibitem[\protect\citeauthoryear{Namkoong and Duchi}{Namkoong and Duchi}{2017}]{namkoong2017variance}
Namkoong, H. and J.~C. Duchi (2017).
\newblock Variance-based regularization with convex objectives.
\newblock {\em Advances in neural information processing systems\/}~{\em 30}.

\bibitem[\protect\citeauthoryear{Pia, Ma, and Tzamos}{Pia et~al.}{2022}]{pmlr-v178-pia22a}
Pia, A.~D., M.~Ma, and C.~Tzamos (2022, 02--05 Jul).
\newblock Clustering with queries under semi-random noise.
\newblock In P.-L. Loh and M.~Raginsky (Eds.), {\em Proceedings of Thirty Fifth Conference on Learning Theory}, Volume 178 of {\em Proceedings of Machine Learning Research}, pp.\  5278--5313. PMLR.

\bibitem[\protect\citeauthoryear{Pidan and El-Yaniv}{Pidan and El-Yaniv}{2011}]{pidan2011selective}
Pidan, D. and R.~El-Yaniv (2011).
\newblock Selective prediction of financial trends with hidden markov models.
\newblock {\em Advances in Neural Information Processing Systems\/}~{\em 24}.

\bibitem[\protect\citeauthoryear{Pollard}{Pollard}{1990}]{pollard1990section}
Pollard, D. (1990).
\newblock Empirical processes.
\newblock Volume~2, pp.\  43--50. Institute of Mathematical Statistics.

\bibitem[\protect\citeauthoryear{Puchkin and Zhivotovskiy}{Puchkin and Zhivotovskiy}{2022}]{puchkin2021exponential}
Puchkin, N. and N.~Zhivotovskiy (2022).
\newblock Exponential savings in agnostic active learning through abstention.
\newblock {\em IEEE Transactions on Information Theory\/}~{\em 68\/}(7), 4651--4665.

\bibitem[\protect\citeauthoryear{Seitzer, Tavakoli, Antic, and Martius}{Seitzer et~al.}{2022}]{seitzer2022on}
Seitzer, M., A.~Tavakoli, D.~Antic, and G.~Martius (2022).
\newblock On the pitfalls of heteroscedastic uncertainty estimation with probabilistic neural networks.
\newblock In {\em International Conference on Learning Representations}.

\bibitem[\protect\citeauthoryear{Shah, Bu, Lee, Das, Panda, Sattigeri, and Wornell}{Shah et~al.}{2022}]{shah2022selective}
Shah, A., Y.~Bu, J.~K. Lee, S.~Das, R.~Panda, P.~Sattigeri, and G.~W. Wornell (2022).
\newblock Selective regression under fairness criteria.
\newblock In {\em International Conference on Machine Learning}, pp.\  19598--19615. PMLR.

\bibitem[\protect\citeauthoryear{Skafte, J{\o}rgensen, and Hauberg}{Skafte et~al.}{2019}]{skafte2019reliable}
Skafte, N., M.~J{\o}rgensen, and S.~Hauberg (2019).
\newblock Reliable training and estimation of variance networks.
\newblock {\em Advances in Neural Information Processing Systems\/}~{\em 32}.

\bibitem[\protect\citeauthoryear{Talagrand}{Talagrand}{1994}]{talagrand1994sharper}
Talagrand, M. (1994).
\newblock Sharper bounds for gaussian and empirical processes.
\newblock {\em The Annals of Probability\/}, 28--76.

\bibitem[\protect\citeauthoryear{Tsybakov}{Tsybakov}{2003}]{tsybakov2003optimal}
Tsybakov, A.~B. (2003).
\newblock Optimal rates of aggregation.
\newblock In {\em Learning Theory and Kernel Machines: 16th Annual Conference on Learning Theory and 7th Kernel Workshop, COLT/Kernel 2003, Washington, DC, USA, August 24-27, 2003. Proceedings}, pp.\  303--313. Springer.

\bibitem[\protect\citeauthoryear{Tsybakov}{Tsybakov}{2004}]{tsybakov2004optimal}
Tsybakov, A.~B. (2004).
\newblock Optimal aggregation of classifiers in statistical learning.
\newblock {\em The Annals of Statistics\/}~{\em 32\/}(1), 135--166.

\bibitem[\protect\citeauthoryear{Valiant}{Valiant}{1984}]{valiant1984theory}
Valiant, L.~G. (1984).
\newblock A theory of the learnable.
\newblock {\em Communications of the ACM\/}~{\em 27\/}(11), 1134--1142.

\bibitem[\protect\citeauthoryear{Van Der~Vaart, Wellner, van~der Vaart, and Wellner}{Van Der~Vaart et~al.}{1996}]{van1996weak}
Van Der~Vaart, A.~W., J.~A. Wellner, A.~W. van~der Vaart, and J.~A. Wellner (1996).
\newblock {\em Weak convergence}.
\newblock Springer.

\bibitem[\protect\citeauthoryear{Vapnik and Chervonenkis}{Vapnik and Chervonenkis}{1974}]{vapnik1974theory}
Vapnik, V. and A.~Chervonenkis (1974).
\newblock Theory of pattern recognition.

\bibitem[\protect\citeauthoryear{Vapnik and Chervonenkis}{Vapnik and Chervonenkis}{1971}]{vapnik1971uniform}
Vapnik, V. and A.~Y. Chervonenkis (1971).
\newblock On the uniform convergence of relative frequencies of events to their probabilities.
\newblock {\em Theory of Probability \& Its Applications\/}~{\em 16\/}(2), 264--280.

\bibitem[\protect\citeauthoryear{Vidyasagar}{Vidyasagar}{2013}]{vidyasagar2013learning}
Vidyasagar, M. (2013).
\newblock {\em Learning and generalisation: with applications to neural networks}.
\newblock Springer Science \& Business Media.

\bibitem[\protect\citeauthoryear{Xie, Ma, and Wang}{Xie et~al.}{2019}]{xie2019towards}
Xie, T., Y.~Ma, and Y.-X. Wang (2019).
\newblock Towards optimal off-policy evaluation for reinforcement learning with marginalized importance sampling.
\newblock {\em Advances in Neural Information Processing Systems\/}~{\em 32}.

\bibitem[\protect\citeauthoryear{Xu and Zeevi}{Xu and Zeevi}{2020}]{xu2020towards}
Xu, Y. and A.~Zeevi (2020).
\newblock Towards optimal problem dependent generalization error bounds in statistical learning theory.
\newblock {\em arXiv preprint arXiv:2011.06186\/}.

\bibitem[\protect\citeauthoryear{Yuan and Wegkamp}{Yuan and Wegkamp}{2010}]{yuan2010classification}
Yuan, M. and M.~Wegkamp (2010).
\newblock Classification methods with reject option based on convex risk minimization.
\newblock {\em Journal of Machine Learning Research\/}~{\em 11\/}(1).

\bibitem[\protect\citeauthoryear{Zhai, Dan, Kolter, and Ravikumar}{Zhai et~al.}{2023}]{zhai2022understanding}
Zhai, R., C.~Dan, J.~Z. Kolter, and P.~K. Ravikumar (2023).
\newblock Understanding why generalized reweighting does not improve over erm.
\newblock In {\em The Eleventh International Conference on Learning Representations}.

\bibitem[\protect\citeauthoryear{Zhang, Lin, Li, Adler, Rasul, Schneider, and Nevmyvaka}{Zhang et~al.}{2023}]{zhang2023risk}
Zhang, Y., J.~Lin, F.~Li, Y.~Adler, K.~Rasul, A.~Schneider, and Y.~Nevmyvaka (2023).
\newblock Risk bounds on aleatoric uncertainty recovery.
\newblock In {\em International Conference on Artificial Intelligence and Statistics}, pp.\  6015--6036. PMLR.

\bibitem[\protect\citeauthoryear{Zhang, Zheng, Dalirrooyfard, Wu, Schneider, Raj, Nevmyvaka, and Chen}{Zhang et~al.}{2023}]{zhang2023learning}
Zhang, Y., S.~Zheng, M.~Dalirrooyfard, P.~Wu, A.~Schneider, A.~Raj, Y.~Nevmyvaka, and C.~Chen (2023).
\newblock Learning to abstain from uninformative data.
\newblock {\em arXiv preprint arXiv:2309.14240\/}.

\bibitem[\protect\citeauthoryear{Zhivotovskiy and Hanneke}{Zhivotovskiy and Hanneke}{2018}]{zhivotovskiy2018localization}
Zhivotovskiy, N. and S.~Hanneke (2018).
\newblock Localization of vc classes: Beyond local rademacher complexities.
\newblock {\em Theoretical Computer Science\/}~{\em 742}, 27--49.

\end{thebibliography}

